A Corpus for Detecting High-Context Medical Conditions in Intensive Care Patient Notes Focusing on Frequently Readmitted Patients

A crucial step within secondary analysis of electronic health records (EHRs) is to identify the patient cohort under investigation. While EHRs contain medical billing codes that aim to represent the conditions and treatments patients may have, much of the information is only present in the patient notes. Therefore, it is critical to develop robust algorithms to infer patients' conditions and treatments from their written notes. In this paper, we introduce a dataset for patient phenotyping, a task that is defined as the identification of whether a patient has a given medical condition (also referred to as clinical indication or phenotype) based on their patient note. Nursing Progress Notes and Discharge Summaries from the Intensive Care Unit of a large tertiary care hospital were manually annotated for the presence of several high-context phenotypes relevant to treatment and risk of re-hospitalization. This dataset contains 1102 Discharge Summaries and 1000 Nursing Progress Notes. Each Discharge Summary and Progress Note has been annotated by at least two expert human annotators (one clinical researcher and one resident physician). Annotated phenotypes include treatment non-adherence, chronic pain, advanced/metastatic cancer, as well as 10 other phenotypes. This dataset can be utilized for academic and industrial research in medicine and computer science, particularly within the field of medical natural language processing.

==> table1-old.tex <==







\begin{table*}[!htb]
\centering

\caption{The ten different phenotypes used for our dataset. The first column shows the name of the phenotype, the second column shows the number of positive examples our of the total 1,610 Discharge summaries, and the third shows the $\kappa$ coefficient as inter-rater agreement measure. The last column lists the definition for each phenotype that was used to identify and annotate the phenotype.}

\label{tab:data}
\begin{tabularx}{\textwidth}{|p{3.5cm}|c|c|X|}
\hline
\textbf{Phenotype}                                   & \textbf{\#pos.} & $\kappa $ & \textbf{Definition}                                   \\ \hline

Adv. / Metastatic Cancer & 161 & 0.83 & Cancers with very high or imminent mortality (pancreas, esophagus, stomach, cholangiocarcinoma, brain); mention of distant or multi-organ metastasis, where palliative care would be considered (prognosis $< 6$ months). \\ \hline

Adv. Heart Disease & 275 & 0.82 & Any consideration for needing a heart transplant; description of severe aortic stenosis (aortic valve area $< 1.0\mathrm{cm}^2$), severe cardiomyopathy, Left Ventricular Ejection Fraction (LVEF) \textless= 30\%. Not sufficient to have a medical history of congestive heart failure (CHF) or myocardial infarction (MI) with stent or coronary artery bypass graft (CABG) as these are too common. \\ \hline

Adv. Lung Disease & 167 &  0.81 & Severe chronic obstructive pulmonary disease (COPD) defined as Gold Stage III-IV, or with a forced expiratory volume during first breath (FEV1) $< 50\%$ of normal, or forced vital capacity (FVC) $< 70\%$, or severe interstitial lung disease (ILD), or Idiopathic pulmonary fibrosis (IPF). \\ \hline

Alcohol Abuse & 196 & 0.86 & Current/recent alcohol abuse history; still an active problem at time of admission (may or may not be the cause of it). \\ \hline

Chronic Neurologic Dystrophies & 368 & 0.71 & Any chronic central nervous system (CNS) or spinal cord diseases, included/not limited to: Multiple sclerosis (MS), amyotrophic lateral sclerosis (ALS), myasthenia gravis, Parkinson’s Disease, epilepsy, history of stroke/cerebrovascular accident (CVA) with residual deficits, and various neuromuscular diseases/dystrophies. \\ \hline

Chronic Pain & 321 & 0.83 & Any etiology of chronic pain, including fibromyalgia, requiring long-term opioid/narcotic analgesic medication to control. \\ \hline
Dementia & TODO & TODO & Alzheimer's, alcohol-associated, and other forms of dementia mentioned in the text. \\ \hline 

Depression & 460 & 0.95 & Diagnosis of depression; prescription of anti-depressant medication; or any description of intentional drug overdose, suicide or self-harm attempts. \\ \hline 

Developmental Delay & TODO & TODO & Includes congenital, genetic and idiopathic disabilities. \\ \hline

Non Adherence & TODO & TODO & Temporary or permanent discontinuation of a treatment, including pharmaceuticals or appointments, without consulting a physician prior to doing so. This includes skipping dialysis appointments or leaving the hospital against medical advice. A patient who sees a physician to discuss adverse events associated with a medication may or may not constitute non-adherence depending on whether or not the treatment was ceased without the physician's consultation. \\ \hline

Obesity & 126 & 0.94 & Clinical obesity. BMI $> 30$. Previous history of or being considered for gastric bypass. Insufficient to have abdominal obesity mentioned in physical exam. \\ \hline

Psychiatric disorders & 295 & 0.91 & All psychiatric disorders in DSM-5 classification, including schizophrenia, bipolar and anxiety disorders, other than depression. \\ \hline

Substance Abuse & 155 & 0.86 & Include any intravenous drug abuse (IVDU), accidental overdose of psychoactive or narcotic medications,(prescribed or not). Admitting to marijuana use in history is not sufficient. \\ \hline

\end{tabularx}
\end{table*}







==> table1.tex <==







\begin{table*}[!htb]
\centering

\caption{The thirteen different phenotypes used for our dataset, as well the definition for each phenotype that was used to identify and annotate the phenotype.}

\label{tab:phenotype-description}
\begin{tabularx}{\textwidth}{|p{3.5cm}|X|}
\hline
\textbf{Phenotype} & \textbf{Definition}   \\ \hline

Adv. / Metastatic Cancer &  Cancers with very high or imminent mortality (pancreas, esophagus, stomach, cholangiocarcinoma, brain); mention of distant or multi-organ metastasis, where palliative care would be considered (prognosis $< 6$ months). \\ \hline

Adv. Heart Disease &  Any consideration for needing a heart transplant; description of severe aortic stenosis (aortic valve area $< 1.0\mathrm{cm}^2$), severe cardiomyopathy, Left Ventricular Ejection Fraction (LVEF) \textless= 30\%. Not sufficient to have a medical history of congestive heart failure (CHF) or myocardial infarction (MI) with stent or coronary artery bypass graft (CABG) as these are too common. \\ \hline

Adv. Lung Disease &  Severe chronic obstructive pulmonary disease (COPD) defined as Gold Stage III-IV, or with a forced expiratory volume during first breath (FEV1) $< 50\%$ of normal, or forced vital capacity (FVC) $< 70\%$, or severe interstitial lung disease (ILD), or Idiopathic pulmonary fibrosis (IPF). \\ \hline

Alcohol Abuse & Current/recent alcohol abuse history; still an active problem at time of admission (may or may not be the cause of it). \\ \hline

Chronic Neurologic Dystrophies &  Any chronic central nervous system (CNS) or spinal cord diseases, included/not limited to: Multiple sclerosis (MS), amyotrophic lateral sclerosis (ALS), myasthenia gravis, Parkinson’s Disease, epilepsy, history of stroke/cerebrovascular accident (CVA) with residual deficits, and various neuromuscular diseases/dystrophies. \\ \hline

Chronic Pain &  Any etiology of chronic pain, including fibromyalgia, requiring long-term opioid/narcotic analgesic medication to control. \\ \hline

Dementia & Alzheimer's, alcohol-associated, and other forms of dementia mentioned in the text. \\ \hline 

Depression &  Diagnosis of depression; prescription of anti-depressant medication; or any description of intentional drug overdose, suicide or self-harm attempts. \\ \hline 

Developmental Delay &  Includes congenital, genetic and idiopathic disabilities. \\ \hline

Non Adherence &  Temporary or permanent discontinuation of a treatment, including pharmaceuticals or appointments, without consulting a physician prior to doing so. This includes skipping dialysis appointments or leaving the hospital against medical advice. A patient who sees a physician to discuss adverse events associated with a medication may or may not constitute non-adherence depending on whether or not the treatment was ceased without the physician's consultation. \\ \hline

Obesity & Clinical obesity. BMI $> 30$. Previous history of or being considered for gastric bypass. Insufficient to have abdominal obesity mentioned in physical exam. \\ \hline

Psychiatric disorders &  All psychiatric disorders in DSM-5 classification, including schizophrenia, bipolar and anxiety disorders, other than depression. \\ \hline

Substance Abuse &  Include any intravenous drug abuse (IVDU), accidental overdose of psychoactive or narcotic medications,(prescribed or not). Admitting to marijuana use in history is not sufficient. \\ \hline

\end{tabularx}
\end{table*}







==> table6-examples.tex <==








\begin{table*}[!htb]
\centering

\caption{Examples for each phenotype.}

\label{tab:phenotype-examples}
\begin{tabularx}{\textwidth}{|p{3.5cm}|X|}
\hline
\textbf{Phenotype} & \textbf{Example}   \\ \hline

Adv. / Metastatic Cancer &  h/o cholangiocarcinoma dx in [DATE] s/p resection, with recent CT showing met cholangiocarcinoma \\ \hline

Adv. Heart Disease &  echo in [DATE] showed EF 30\% \\ \hline

Adv. Lung Disease & Pt has significant obstructive and restrictive pulmonary disease, on home oxygen. \\ \hline

Alcohol Abuse & Current/recent alcohol abuse history; still an active problem at time of admission (may or may not be the cause of it). \\ \hline

Chronic Neurologic Dystrophies &  Any chronic central nervous system (CNS) or spinal cord diseases, included/not limited to: Multiple sclerosis (MS), amyotrophic lateral sclerosis (ALS), myasthenia gravis, Parkinson’s Disease, epilepsy, history of stroke/cerebrovascular accident (CVA) with residual deficits, and various neuromuscular diseases/dystrophies. \\ \hline

Chronic Pain &  Any etiology of chronic pain, including fibromyalgia, requiring long-term opioid/narcotic analgesic medication to control. \\ \hline

Dementia & Alzheimer's, alcohol-associated, and other forms of dementia mentioned in the text. \\ \hline 

Depression &  Diagnosis of depression; prescription of anti-depressant medication; or any description of intentional drug overdose, suicide or self-harm attempts. \\ \hline 

Developmental Delay &  Includes congenital, genetic and idiopathic disabilities. \\ \hline

Non Adherence &  Temporary or permanent discontinuation of a treatment, including pharmaceuticals or appointments, without consulting a physician prior to doing so. This includes skipping dialysis appointments or leaving the hospital against medical advice. A patient who sees a physician to discuss adverse events associated with a medication may or may not constitute non-adherence depending on whether or not the treatment was ceased without the physician's consultation. \\ \hline

Obesity & Clinical obesity. BMI $> 30$. Previous history of or being considered for gastric bypass. Insufficient to have abdominal obesity mentioned in physical exam. \\ \hline

Psychiatric disorders &  All psychiatric disorders in DSM-5 classification, including schizophrenia, bipolar and anxiety disorders, other than depression. \\ \hline

Substance Abuse &  Include any intravenous drug abuse (IVDU), accidental overdose of psychoactive or narcotic medications,(prescribed or not). Admitting to marijuana use in history is not sufficient. \\ \hline

\end{tabularx}
\end{table*}






